Gradual Session Types

Session types are a rich type discipline, based on linear types, that lifts the sort of safety claims that come with type systems to communications. However, web-based applications and microservices are often written in a mix of languages, with type disciplines in a spectrum between static and dynamic typing. Gradual session types address this mixed setting by providing a framework which grants seamless transition between statically typed handling of sessions and any required degree of dynamic typing. We propose Gradual GV as a gradually typed extension of the functional session type system GV. Following a standard framework of gradual typing, Gradual GV consists of an external language, which relaxes the type system of GV using dynamic types, and an internal language with casts, for which operational semantics is given, and a cast-insertion translation from the former to the latter. We demonstrate type and communication safety as well as blame safety, thus extending previous results to functional languages with session-based communication. The interplay of linearity and dynamic types requires a novel approach to specifying the dynamics of the language.

==> fig-ggv-reductions.tex <==
\begin{figure}[t]
Structural congruence \hfill \fbox{$P \equiv Q$} 
  \begin{align*}
    ((\nu \alpha)P) \PAR Q &\equiv (\nu \alpha)(P \PAR Q) &
    (\nu \alpha)\proc{()} &\equiv \proc{()}
  \end{align*}  

Expression reduction \boxedrel{e \reduces f}
  \begin{align*}
    v \colon \DYN \Cast{p} \DYN &\reduces v \\
    v \colon \DC \Cast{p} \DC &\reduces v \\
    v \colon \unitk \Cast{p} \unitk &\reduces v \\
    v \colon T \Cast{p} \DYN &\reduces
      (v \colon T \Cast{p} \GroundT) \colon \GroundT \Cast{p} \DYN& 
      \rtext{if $T \neq \DYN$, $T \neq \GroundT$, $T \sim \GroundT$} \\
    v \colon \DYN \Cast{p} T &\reduces
      (v \colon \DYN \Cast{p} \GroundT) \colon \GroundT \Cast{p} T& 
      \rtext{if $T \neq \DYN$, $T \neq \GroundT$, $T \sim \GroundT$} \\
    (v \colon \GroundT \Cast{p} \DYN) \colon \DYN \Cast{q} \GroundU &\reduces
       v &
       \rtext{if $\GroundT \lesssim \GroundU$} \\
    (v \colon \GroundT \Cast{p} \DYN) \colon \DYN \Cast{q} \GroundU &\reduces
       \blame{q}&
       \rtext{if $\GroundT \lnsim \GroundU$} \\
    (v \colon T \to_\Multm U \Cast{p} T' \to_\Multn U')\,w &\reduces
      v\, (w \colon T' \Cast{\dual p} T) \colon U \Cast{p} U' \\
    (v,w)_\Multm \colon T \tcpair_\Multm U \Cast{p} T' \tcpair_\Multn U' &\reduces
      (v \colon T \Cast{p} T', w \colon U \Cast{p} U')_\Multn \\
    \send{v}{(w \colon \pl{T}S \Cast{p} \pl{T'}S')} &\reduces
      (\send{(v \colon T' \Cast{\dual p} T)}{w}) \colon S \Cast{p} S' \\
    \recv (w \colon \qu{T}S \Cast{p} \qu{T'}S') &\reduces
       (\recv w) \colon T \tcpair_\lin S \Cast{p} T' \tcpair_\lin S' \\
       % \letin{y,z}{\recv w}{(y \colon T \Cast{p} T', z \colon S \Cast{p} S')_\lin} \\
    \select{l_j}{(w \colon \oplus\br{l_i\colon S_i}_{i\in I} \Cast{p}
       \oplus\br{l_i\colon S'_i}_{i\in J})} &\reduces
       (\select{l_j}{w}) \colon S_j \Cast{p} S_j'&
       \rtext{if $j \in J$, $J \subseteq I$} \\
    \case{(w \colon \with\br{l_i\colon S_i}_{i\in I} \Cast{p} \with\br{l_i\colon S'_i}_{i\in J})}
        {\br{\casebranch{l_i}{x_i}{e_i}}_{i \in J}} &\reduces
        \case{w}{\br{\casebranch{l_i}{x_i}{\letin{x_i}{(x_i \colon S_i \Cast{p} S_i')}{e_i}}}_{i \in I}}&
        \text{if $I \subseteq J$} \\
    \close{(v \colon \Endpl \Cast{p} \Endpl)} &\reduces \close{v}\\
    \wait{(v \colon \Endqu \Cast{p} \Endqu)} &\reduces \wait{v}
  \end{align*}
  \spacer

Process reduction  \hfill \fbox{$P \reduces Q$}
  \begin{align}
    \proc{ \contextE{w \colon \GroundT \Cast{p} \DYN} } &\reduces
      (\nu\alpha)(\proc{\context{\alpha}} \PAR \alpha\mapsto\wrap[p]{w}{\GroundT})&
      \rtext{if $\lin(\GroundT)$} \\
    \proc{ \contextE{\alpha \colon \DYN \Cast{q} \GroundU} }
      \PAR \alpha \mapsto \wrap[p]{w}{\GroundT} &\reduces
      \proc{ \contextE{(\wrap[p]{w}{\GroundT}) \colon \DYN \Cast{q} \GroundU} }
      \PAR \alpha\mapsto\locked & 
      \rtext{if $\lin(\GroundT)$}\\
    \proc{ \contextE{\alpha \colon \DYN \Cast{p} \GroundU} }
      \PAR \alpha \mapsto \locked &\reduces
      \proc {\contextE{\blame{p}}} \\
    (\nu\alpha) ( \alpha \mapsto \wrap[p]{w}{\GroundT} ) &\reduces
      (\nu\alpha) ( \alpha \mapsto \wrap[p]w{\GroundT} \PAR \proc{\blame{\dual{p}}} )&
      \rtext{if $\lin(\GroundT)$} \\      
    \proc{ \contextE{w \colon S \Cast{p} \DC} } &\reduces
      \proc{ \contextE{(w \colon S \Cast{p} \GroundS) \colon \GroundS \Cast{p} \DC} } &
      \rtext{if $S \ne \DC$, $S \ne \GroundS$, $S \sim \GroundS$} \\
    \proc{ \contextE{w \colon \DC \Cast{p} S} } &\reduces
      \proc{ \contextE{(w \colon \DC \Cast{p} \GroundS ) \colon \GroundS \Cast{p} S} }&
      \rtext{if $S \ne \DC$, $S \ne \GroundS$, $S \sim \GroundS$} \\
    \proc{ \contextE{(w \colon \GroundS \Cast{p} \DC)  \colon \DC \Cast{q} \GroundR} } &\reduces
      \proc{ \contextE{w} } &
      \rtext{if $\GroundS \lesssim  \GroundR$}\\
    \proc{ \contextE{(w \colon \GroundS \Cast{p} \DC)  \colon \DC \Cast{q} \GroundR} } &\reduces
      \proc{ \contextE{(w \colon \GroundS \Cast{p} \DC)  \colon \DC \Cast{q} \GroundR} }
      \PAR \proc{\blame{\dual{p}}} \PAR \proc{\blame{q}} &
      \rtext{if $\GroundS \lnsim \GroundR$} \\
    (\nu c,d)( \proc{ \contextE{\Chanc \colon \DC \Cast{p} \GroundS} }
               \PAR \proc{ \contextF{\Chand \colon \DC \Cast{q} {\GroundR}} }) &\reduces
      (\nu c,d)( \proc{ \contextE{\Chanc} } \PAR \proc{ \contextF{\Chand } })
      &\rtext{if $\dual{\GroundS} \lesssim {\GroundR}$}
      \label{redn:channel-cancel} \\
    (\nu c,d)( \proc{ \contextE{\Chanc \colon \DC \Cast{p} \GroundS} }
               \PAR \proc{ \contextF{\Chand \colon \DC \Cast{q} \GroundR} }) &\reduces
      (\nu c,d)( \proc{ \contextE{\Chanc} } \PAR \proc{ \contextF{\Chand} }\label{redn:channel-blame}
                 \PAR \proc{\blame{p}} \PAR \proc{\blame{q}} )&
      \text{if $\dual{\GroundS} \lnsim \GroundR$}
  \end{align}

 \hcaption{Reduction in \GGV}
 \label{fig:ggv-reductions-expressions}
\end{figure}




==> quote-setup.tex <==
\usepackage{framed}
\usepackage{xcolor}
\let\oldquote=\quote
\let\endoldquote=\endquote
\colorlet{shadecolor}{orange!15}
\renewenvironment{quote}{\begin{shaded*}\begin{oldquote}}{\end{oldquote}\end{shaded*}}


==> texdirectives.tex <==
 


==> tsuda/figures/alg-tycheck-proc.tex <==
%% Typechecking algorithm for processes

\begin{algorithmic}
%%  \Require {A type environment $\Gamma$ and a process $P$}
%%  \Ensure {The set of used linear variables in typing}
%%  assertion fails if not typable

  \Function{\typroc}{$\Gamma, P$}
    \Case{$P$}
      \CaseItem{$ \proc{  \mathbb{e}  } $}
        \State $T, X \asgn$ \Call{\tyexp}{$\Gamma, e$}
        \State \Assert $\un(T)$
        \State \Return $X$
      \EndCaseItem

      \CaseItem{$( \ottnt{P_{{\mathrm{1}}}}  \PAR  \ottnt{P_{{\mathrm{2}}}} )$}
        \State $X \asgn$ \Call{\typroc}{$\Gamma, P_1$}
        \State $Y \asgn$ \Call{\typroc}{$\Gamma, P_2$}
        %% ASSERT_DISJOINT
        \State \Assert $X \cap Y = \emptyset$

        \State \Return $X \cup Y$
      \EndCaseItem

      \CaseItem{$ ( \nu   \ottmv{c} {:} \ottnt{S} ,  \ottmv{d} )  \ottnt{P_{{\mathrm{1}}}} $}
        \State $\Gamma' \asgn \Gamma  \ottsym{,}  \ottmv{c}  \ottsym{:}  \ottnt{S}  \ottsym{,}  \ottmv{d}  \ottsym{:}   \dual{  \ottnt{S}  } $
        \State $X \asgn$ \Call{\typroc}{$\Gamma', P_1$}

        %% c, d is linear
        \State \Assert $c \in X$ and $d \in X$
        \State \Return $X \setminus \set{c,d}$
      \EndCaseItem
    \EndCase
  \EndFunction
\end{algorithmic}


==> tsuda/figures/polarized-subtyping.tex <==
\begin{figure}[t]
  Polarised consistent subtyping\hfill\fbox{$\texttt{\textcolor{red}{<<no parses (char 5):  T <<***+ U  >>}} \quad \texttt{\textcolor{red}{<<no parses (char 5):  T <<***- U  >>}}$}
  \\
  Polarities $\ottnt{u}$ range over $ \oplus ,  \ominus $;
  complemented by the flip operation: $ \overline{  \oplus  }  =  \ominus $ and  $ \overline{  \ominus  }  =  \oplus $
  \begin{mathpar}
    \inferrule{}{
      \texttt{\textcolor{red}{<<no parses (char 7):  dyn <<***+ U  >>}}
    }

    \inferrule{}{
      \texttt{\textcolor{red}{<<no parses (char 5):  T <<***- dyn  >>}}
    }

    \inferrule{}{
      \texttt{\textcolor{red}{<<no parses (char 8):  unit <<***u unit  >>}}
    }
    \\
    \inferrule{
      \texttt{\textcolor{red}{<<no parses (char 5):  T <<***u T'  >>}} \andalso
      \texttt{\textcolor{red}{<<no parses (char 5):  U <<***u U'  >>}} \andalso
      \ottnt{m}  \Sub  \ottnt{n}
    }{
      \texttt{\textcolor{red}{<<no parses (char 12):  (T *m U) <<***u (T' *n U')  >>}}
    }
    
    \inferrule{
      \texttt{\textcolor{red}{<<no parses (char 6):  T' <<*** (flip u) T  >>}} \andalso
      \texttt{\textcolor{red}{<<no parses (char 5):  U <<***u U'  >>}} \andalso
      \ottnt{m}  \Sub  \ottnt{n}
    }{
      \texttt{\textcolor{red}{<<no parses (char 13):  (T ->m U) <<***u (T' ->n U')  >>}}
    }
    \\
    \inferrule{}{
      \texttt{\textcolor{red}{<<no parses (char 6):  dc <<***+ R  >>}}
    }
    
    \inferrule{}{
      \texttt{\textcolor{red}{<<no parses (char 5):  S <<***- dc  >>}}
    }
    
    \inferrule{}{
      \texttt{\textcolor{red}{<<no parses (char 8):  end! <<***u end!  >>}}
    }
    
    \inferrule{}{
      \texttt{\textcolor{red}{<<no parses (char 8):  end\mbox{?} <<***u end\mbox{?}  >>}}
    }
    \\
    \inferrule{
      \texttt{\textcolor{red}{<<no parses (char 6):  T' <<*** (flip u) T  >>}} \andalso
      \texttt{\textcolor{red}{<<no parses (char 5):  S <<***u S'  >>}}      
    }{
      \texttt{\textcolor{red}{<<no parses (char 8):  !T.S <<***u !T'.S'  >>}}
    }
    
    \inferrule{
      \texttt{\textcolor{red}{<<no parses (char 5):  T <<***u T'  >>}} \andalso
      \texttt{\textcolor{red}{<<no parses (char 5):  S <<***u S'  >>}} \andalso
    }{
      \texttt{\textcolor{red}{<<no parses (char 8):  \mbox{?}T.S <<***u \mbox{?}T'.S'  >>}}
    }
    \\
    \inferrule{
      \texttt{\textcolor{red}{<<no parses (char 6):  Sj <<***u Rj  >>}} \andalso j \in J \subseteq I
    }{
      \texttt{\textcolor{red}{<<no parses (char 23):  (+)\{li:Si \mbox{$\mid$} i in I\} <<***u (+)\{lj:Rj \mbox{$\mid$} j in J\}  >>}}
    }
    
    \inferrule{
      \texttt{\textcolor{red}{<<no parses (char 6):  Si <<***u Ri  >>}} \andalso i \in I \subseteq J
    }{
      \texttt{\textcolor{red}{<<no parses (char 21):  \&\{li:Si \mbox{$\mid$} i in I\} <<***u \&\{lj:Rj \mbox{$\mid$} j in J\}  >>}}
    }
  \end{mathpar}
  \hcaption{Polarised consistent subtyping.}
  \label{fig:polarised-consistent-subtyping}
\end{figure}

